Does spontaneous motion lead to intuitive Body-Machine Interfaces? A fitness study of different body segments for wearable telerobotics

Human-Robot Interfaces (HRIs) represent a crucial component in telerobotic systems. Body-Machine Interfaces (BoMIs) based on body motion can feel more intuitive than standard HRIs for naive users as they leverage humans' natural control capability over their movements. Among the different methods used to map human gestures into robot commands, data-driven approaches select a set of body segments and transform their motion into commands for the robot based on the users' spontaneous motion patterns. Despite being a versatile and generic method, there is no scientific evidence that implementing an interface based on spontaneous motion maximizes its effectiveness. In this study, we compare a set of BoMIs based on different body segments to investigate this aspect. We evaluate the interfaces in a teleoperation task of a fixed-wing drone and observe users' performance and feedback. To this aim, we use a framework that allows a user to control the drone with a single Inertial Measurement Unit (IMU) and without prior instructions. We show through a user study that selecting the body segment for a BoMI based on spontaneous motion can lead to sub-optimal performance. Based on our findings, we suggest additional metrics based on biomechanical and behavioral factors that might improve data-driven methods for the design of HRIs.

==> operators.tex <==
% THIS FILE NEEDS TO BE IMPROVED A LOT (ORGANIZATION AND CONTENT)

%Spaces
\newcommand{\real}[1]{\mathbb{R}^{#1}{}}
\newcommand{\complex}[1]{\mathbb{C}^{#1}{}}
\newcommand{\naturals}[1]{\mathbb{N}^{#1}{}}
\newcommand{\integers}[1]{\mathbb{Z}^{#1}{}}
\newcommand{\sphere}[1]{{\mathbb{S}^{#1}}{}}
\newcommand{\stiefel}{\mathrm{St}}
\newcommand{\grassmann}{\mathrm{Grass}}
\newcommand{\GL}{\mathbb{GL}}

%short-hand for matrices
\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\Bmat}[1]{\begin{Bmatrix}#1\end{Bmatrix}}
\newcommand{\pmat}[1]{\begin{pmatrix}#1\end{pmatrix}}

%supertscript operators
\newcommand{\transpose}{^\mathrm{T}}
\newcommand{\hermitian}{^\mathrm{H}}
\newcommand{\inverse}{^{-1}}
\newcommand{\pinverse}{^\dagger}
\newcommand{\orth}{^{\bot}}
\newcommand{\apstar}{^{\ast}}

%parentheses-based operators
\newcommand{\cross}[1]{[#1]_{\times}\!}
\newcommand{\crossinv}[1]{[#1]_{\times}^{\textrm{inv}}\!}

%equality
\newcommand{\defeq}{\doteq}


%Norms, absolute values, and inner products
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\bigabs}[1]{\bigl\lvert#1\bigr\rvert}
\newcommand{\ceil}[1]{\lceil#1\rceil}
\newcommand{\bigceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\bignorm}[1]{\left\lVert#1\right\rVert}
\newcommand{\frob}[1]{\norm{#1}_F}
\newcommand{\bigfrob}[1]{\bignorm{#1}_F}
\newcommand{\metric}[2]{\langle #1, #2\rangle}

%Derivatives
\newcommand{\de}{\mathrm{d}}
\newcommand{\dert}[1][]{\frac{\de #1}{\de t}}
\newcommand{\ddert}[1][]{\frac{\de^2 #1}{\de t^2}}
%Vector
\newcommand{\vct}[1]{\mathbf{#1}}
\newcommand{\pder}[2][]{\frac{\partial #1}{\partial #2}}
%named operators
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\nullsp}{null}
\DeclareMathOperator{\nullity}{nullity}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\blkdiag}{blkdiag}
\DeclareMathOperator{\symm}{sym}
\DeclareMathOperator{\asym}{skew}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\vecspan}{span}
\DeclareMathOperator{\vecop}{vec}
\DeclareMathOperator{\stack}{stack}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\expm}{expm}

\DeclareMathOperator{\grad}{{grad}}
\DeclareMathOperator{\D}{D\!}
\DeclareMathOperator{\Dgrad}{{Dgrad}}
\DeclareMathOperator{\hess}{{Hess}}

\DeclareMathOperator*{\inj}{inj}
\DeclareMathOperator{\hull}{hull}

\DeclareMathOperator{\proj}{{proj}}

\DeclareMathOperator*{\logm}{logm}
\DeclareMathOperator{\Log}{Log}
\DeclareMathOperator{\LogNorm}{\frac{Log}{\norm{Log}}}
\DeclareMathOperator{\DLog}{DLog}
\DeclareMathOperator{\DLogNorm}{D\frac{Log}{\norm{Log}}}

\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\cvxhull}{co}

\DeclareMathOperator{\dist}{dist}

\DeclareMathOperator*{\bigO}{O}

%text for constrained optimization
\newcommand{\subjectto}{\textrm{subject to }}

%%% Local Variables: 
%%% mode: latex
%%% End: 


